Natural Posterior Network: Deep Bayesian Uncertainty for Exponential Family Distributions

Uncertainty awareness is crucial to develop reliable machine learning models. In this work, we propose the Natural Posterior Network (NatPN) for fast and high-quality uncertainty estimation for any task where the target distribution belongs to the exponential family. Thus, NatPN finds application for both classification and general regression settings. Unlike many previous approaches, NatPN does not require out-of-distribution (OOD) data at training time. Instead, it leverages Normalizing Flows to fit a single density on a learned low-dimensional and task-dependent latent space. For any input sample, NatPN uses the predicted likelihood to perform a Bayesian update over the target distribution. Theoretically, NatPN assigns high uncertainty far away from training data. Empirically, our extensive experiments on calibration and OOD detection show that NatPN delivers highly competitive performance for classification, regression and count prediction tasks.

==> include/xx-checklist.tex <==
\section*{Checklist}
% \answerTODO{}
% \answerNO{}
% \answerYES{}
% \answerNA{}

\begin{enumerate}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Sec.~\ref{sec:limitations}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Sec.~\ref{sec:broader-impact}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Thm.~\ref{thm:oodom-guarantee} and Sec. \emph{Proofs} in App.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See Sec. \emph{Proofs} in App.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Sec.~\emph{Models Details} in App.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Sec.~\emph{Models Details} and Sec.~\emph{Datasets Details} in App.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
   \answerYes{See Sec.~\ref{sec:experiments}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Sec.~\emph{Models Details} in App.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite the original papers and sources presenting the used datasets.}
  \item Did you mention the license of the assets?
    \answerYes{We provided the license of the datasets when available. See Sec.~\emph{Datasets Details} in App.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We provide code for the new model. See Sec.~\emph{Models Details} in App.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> tables/auroc-Kin8nm.tex <==
\begin{table*}[ht]
    \caption{Kin8nm AUC-ROC}
    \centering
    \scriptsize
    \begin{tabular}{lcccccc}
        \toprule
        & \textbf{Energy Alea.} & \textbf{Energy Epist.} & \textbf{Concrete Alea.} & \textbf{Concrete Epist.} & \textbf{Kin8nm Alea.} & \textbf{Kin8nm Epist.} \\
        \midrule
        \textbf{Dropout} & 93.24 $\pm$ 5.19 & 99.96 $\pm$ 0.04 & *100.00 $\pm$ 0.00 & *100.00 $\pm$ 0.00 & *100.00 $\pm$ 0.00 & *100.00 $\pm$ 0.00 \\
        \textbf{Ensemble} & *100.00 $\pm$ 0.00 & *100.00 $\pm$ 0.00 & *100.00 $\pm$ 0.00 & *100.00 $\pm$ 0.00 & *100.00 $\pm$ 0.00 & *100.00 $\pm$ 0.00 \\
        \midrule
        \textbf{EvReg} & 80.00 $\pm$ 20.00 & 80.00 $\pm$ 20.00 & \textbf{*100.00 $\pm$ 0.00} & 80.00 $\pm$ 20.00 & \textbf{*100.00 $\pm$ 0.00} & \textbf{*100.00 $\pm$ 0.00} \\
        \textbf{\oursacro{}} & \textbf{*100.00 $\pm$ 0.00} & \textbf{*100.00 $\pm$ 0.00} & \textbf{*100.00 $\pm$ 0.00} & \textbf{*100.00 $\pm$ 0.00} & \textbf{*100.00 $\pm$ 0.00} & \textbf{*100.00 $\pm$ 0.00} \\
        \bottomrule
    \end{tabular}
\end{table*}

==> tables/auroc-concrete.tex <==
\begin{table*}[ht]
    \caption{Concrete AUC-ROC}
    \centering
    \scriptsize
    \begin{tabular}{lcccccc}
        \toprule
        & \textbf{Energy Alea.} & \textbf{Energy Epist.} & \textbf{Concrete Alea.} & \textbf{Concrete Epist.} & \textbf{Kin8nm Alea.} & \textbf{Kin8nm Epist.} \\
        \midrule
        \textbf{Dropout} & 7.07 $\pm$ 4.83 & 99.31 $\pm$ 0.20 & 11.02 $\pm$ 7.95 & 99.17 $\pm$ 0.28 & 11.02 $\pm$ 7.95 & 99.17 $\pm$ 0.28 \\
        \textbf{Ensemble} & 58.04 $\pm$ 18.97 & *100.00 $\pm$ 0.00 & 73.40 $\pm$ 19.43 & *100.00 $\pm$ 0.00 & 73.40 $\pm$ 19.43 & *100.00 $\pm$ 0.00 \\
        \midrule
        \textbf{EvReg} & 1.08 $\pm$ 1.03 & 58.35 $\pm$ 18.18 & 0.00 $\pm$ 0.00 & 34.00 $\pm$ 21.23 & 0.00 $\pm$ 0.00 & 34.00 $\pm$ 21.23 \\
        \textbf{\oursacro{}} & \textbf{*100.00 $\pm$ 0.00} & \textbf{*100.00 $\pm$ 0.00} & \textbf{*100.00 $\pm$ 0.00} & \textbf{*100.00 $\pm$ 0.00} & \textbf{*100.00 $\pm$ 0.00} & \textbf{*100.00 $\pm$ 0.00} \\
        \bottomrule
    \end{tabular}
\end{table*}

==> tables/auroc-nyu.tex <==
\begin{table*}[ht]
    \caption{NYU AUC-ROC}
    \centering
    \scriptsize
    \begin{tabular}{lcccccccc}
        \toprule
        & \textbf{LSUN Alea. Cl} & \textbf{LSUN Alea. Ch} & \textbf{LSUN Epist. Cl} & \textbf{LSUN Epist. Ch} & \textbf{Kitti Alea.} & \textbf{Kitti Epist.} & \textbf{OODom Alea.} & \textbf{OODom Epist.} \\
        \midrule
        \textbf{Dropout} & *85.68 & 92.20 & 58.10 & 56.51 & 93.35 & 60.31 & 61.47 & *100.00 \\
        \midrule
        \textbf{EvReg} & 8.00 & 3.15 & 24.76 & 14.45 & 2.45 & 11.97 & 45.75 & 1.19 \\
        \textbf{\oursacro{}} & \textbf{83.75} & \textbf{*95.97} & \textbf{*64.63} & \textbf{*72.97} & \textbf{*97.18} & \textbf{*83.15} & \textbf{*100.00} & \textbf{*100.00} \\
        \bottomrule
    \end{tabular}
\end{table*}


==> tables/auroc-sensorlessdrive.tex <==
\begin{table*}[ht]
    \caption{Sensorless Drive AUC-ROC}
    \centering
    \scriptsize
    \begin{tabular}{lcccc}
        \toprule
        & \textbf{9/10 Alea.} & \textbf{9/10 Epist.} & \textbf{OODom Alea.} & \textbf{OODom Epist.} \\
        \midrule
        \textbf{Dropout} & 22.08 $\pm$ 2.31 & 39.90 $\pm$ 3.59 & 3.47 $\pm$ 0.52 & 99.06 $\pm$ 0.38 \\
        \textbf{Ensemble} & 24.30 $\pm$ 1.33 & 37.54 $\pm$ 1.89 & 3.59 $\pm$ 0.59 & 99.95 $\pm$ 0.01 \\
        \textbf{NatPE} & *91.77 $\pm$ 1.27 & 79.61 $\pm$ 2.96 & 99.97 $\pm$ 0.00 & *100.00 $\pm$ 0.00 \\
        \midrule
        \textbf{R-PriorNet} & 54.79 $\pm$ 5.47 & 32.17 $\pm$ 2.50 & \textbf{*100.00 $\pm$ 0.00} & 0.01 $\pm$ 0.00 \\
        \textbf{EnD$^2$} & 19.25 $\pm$ 2.72 & 11.40 $\pm$ 2.30 & 79.57 $\pm$ 19.89 & 0.00 $\pm$ 0.00 \\
        \textbf{PostNet} & 86.22 $\pm$ 1.41 & \textbf{*94.10 $\pm$ 0.99} & 99.99 $\pm$ 0.00 & 99.99 $\pm$ 0.00 \\
        \textbf{\oursacro{}} & \textbf{89.21 $\pm$ 1.91} & 83.51 $\pm$ 3.93 & 99.96 $\pm$ 0.00 & \textbf{*100.00 $\pm$ 0.00} \\
        \bottomrule
    \end{tabular}
\end{table*}


==> tables/tinyimagenet.tex <==
\begin{table*}[ht]
    \centering
    \scriptsize
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{lcccccccc}
        \toprule
        & \textbf{Accuracy} & \textbf{Brier} & \textbf{SVHN Alea.} & \textbf{SVHN Epist.} & \textbf{CelebA Alea.} & \textbf{CelebA Epist.} & \textbf{OODom Alea.} & \textbf{OODom Epist.} \\
        \midrule
        \textbf{Ensemble} & *73.98 & *40.87 & *77.08 & 15.91 & *70.90 & 17.15 & 8.89 & 99.87 \\
        \midrule
        \textbf{PostNet} & 60.30 & \textbf{56.47} & 68.51 & \textbf{*57.54} & 55.57 & \textbf{*37.38} & 99.87 & 99.87 \\
        \textbf{\oursacro{}} & \textbf{63.74} & 59.24 & \textbf{70.84} & 22.84 & \textbf{58.13} & 17.08 & \textbf{*99.91} & \textbf{*99.93} \\
        \bottomrule
    \end{tabular}
    }
    \caption{Results on Tiny-ImageNet (classification with Categorical target distribution). Best scores among all single-pass models are in bold. Best scores among all models are starred. Gray numbers indicate that R-PriorNet has seen samples from the FMNIST dataset during training.}
    \label{tab:mnist}
            \vspace{-.3cm}
\end{table*}
